Thinking with Video: Video Generation as a Promising Multimodal Reasoning Paradigm

The "Thinking with Text" and "Thinking with Images" paradigms significantly improve the reasoning abilities of large language models (LLMs) and Vision-Language Models (VLMs). However, these paradigms have inherent limitations. (1) Images capture only single moments and fail to represent dynamic processes or continuous changes, and (2) The separation of text and vision as distinct modalities, which hinders unified multimodal understanding and generation. Therefore, we propose "Thinking with Video", a new paradigm that leverages video generation models such as Sora-2 to use video frames as a unified medium for multimodal reasoning. To support this exploration, we developed the Video Thinking Benchmark (VideoThinkBench), which covers both vision-centric tasks (e.g., Eyeballing Puzzles) and text-centric tasks (e.g., GSM8K and MMMU). Our evaluation on VideoThinkBench establishes Sora-2 as a capable reasoner. On vision-centric tasks, Sora-2 is comparable to state-of-the-art (SOTA) VLMs, and even surpasses GPT-5 by 10% on eyeballing puzzles. On text-centric tasks, Sora-2 achieves 92% accuracy on MATH, and 69.2% accuracy on MMMU. Furthermore, we systematically analyze the source of these abilities. We also find that self-consistency and in-context learning can improve Sora-2's performance. In summary, our findings show that the video generation model is the potential unified multimodal understanding and generation model, positioning "Thinking with Video" as a potential unified multimodal reasoning paradigm.

==> old/section/evaluation/b_vision.tex <==
\begin{figure*}[!t]
\centering 
\includegraphics[width=\textwidth]{img/eyeballing.pdf}
\caption{\textbf{Four Examples of Sora-2 solving our custom benchmark of 21 eyeballing tasks and 1050 samples.} Each sample is a multiple choice question and includes an input image with text prompt. The benchmark is automatically evaluated and verifiable. See Section~\ref{sec:spatial_reasoning} for details and prompts. In the bottom two examples, Sora-2 adds ``Charlie'' text on options that are not ``C''. This disparity between modalities is further explored in Section~\ref{sec:output_form}. All prompts can be found in Section~\ref{appendix_sec:eyeballing_prompts}.}
\label{fig:case_ray}
\end{figure*}

\subsection{Vision-Centric Reasoning}
\label{sec:eval_mmknowledge}

\subsubsection{Eyeballing Puzzles: Sora-2 exhibits geometric and physical reasoning abilities}
\label{sec:spatial_reasoning}
\textbf{Dataset Construction}

\textit{The eyeballing game}\footnote{https://woodgears.ca/eyeball/} is a game that tests a player's ability to precisely \textbf{estimate geometric properties}. For example, the ``midpoint'' challenge asks player to drag the movable point to the midpoint of two fixed points.

As shown in Fig.~\ref{fig:case_ray}, we manually designed \textbf{21 tasks of verifiable eyeballing puzzles} to test spatial reasoning ability of Sora-2 and VLMs, each puzzle involving a distinct geometry concept. The input of a puzzle instance is an image and a prompt. Every puzzle is in multiple choices form, and can be automatically generated and evaluated. For the following evaluation, we generated 50 samples for each task, which is \textbf{1050 samples in total}. Detailed information of 21 puzzles can be found in Section~\ref{appendix_sec:eyeballing_overview}.

We divide 21 eyeballing tasks into 3 categories: Point Task, Line Task and Shape Task. Accuracy of each category is shown in Table \ref{tab:spatial_reasoning_results}. Point Task constructs a point, such as incenter of a triangle. Line Task constructs a line, such as an angle bisector line. Shape Task constructs a shape, such as given three vertices, finding the fourth vertex to construct a parallelogram. 

\textbf{Evaluation Setup}

For Sora-2, since it generates both video and audio, multiple evaluation methods can be used on it. The evaluation methods of Sora-2 on Eyeballing Puzzles are introduced as follows:
\begin{itemize}
    \item \textbf{Audio Evaluation:} The prompt instructs model to speak out the option in phonetic alphabet (``Alpha'', ``Bravo'', ``Charlie'', ``Delta'' and ``Echo''). Audio is extracted from generated video and transcribed using whisper-1 model. Then a program finds first appearing phonetic alphabet word as the audio option. Finally, Compare the audio option with ground truth.
    
    \item \textbf{Last Frame Evaluation:} The prompt instructs model to draw a red dot on correct option. The last frame of generated video is fed to an image evaluator program that calculates average coordination of red pixels. The last frame option is the option nearest to average coordination of red pixels, or none if there are no red pixels found. Finally, Compare the last frame option with ground truth.
    
    \item \textbf{Major Frame Evaluation:} For every 5 frames in the video, one frame is extracted and fed to the image evaluator, getting option of this frame. Major frame option is the majority vote result of all chosen frames. ``None'' option is excluded from voting. Finally, Compare the Major frame option with ground truth.
\end{itemize}

For VLMs, they are instructed to include chosen option in its response, and a program will extract it. Their prompts are different from Sora-2's, not instructing about drawing. For example, the prompt of Ray Intersection puzzle for VLMs is: \textit{``Which option is the intersection point of the three lines? Answer an option in A-E.``}

\textbf{Evaluation Results}

The correctness rates for Sora-2 and three leading VLMs are presented in Table~\ref{tab:spatial_reasoning_results}. Our analysis focuses on Sora-2's performance across its output modalities and its comparison against other models.

First, leveraging Sora-2's video output proves most effective. The \textbf{Major Frame Evaluation}, which aggregates information across multiple frames, achieves the highest average correctness of \textbf{40.2\%}. This significantly outperforms both the \textbf{Last Frame Evaluation (33.4\%)} and the \textbf{Audio Evaluation (28.0\%)}, demonstrating that the temporal consistency of video provides a more robust measure of its reasoning. A deeper analysis of these output forms is in Section~\ref{sec:output_form}.

When compared to other VLMs, Sora-2's video-based performance stands out. Its \textbf{40.2\%} average score \textbf{surpasses all competitors}, including \textbf{Claude 4.5 (35.1\%)}, \textbf{GPT5-high (29.7\%)}, and \textbf{Gemini 2.5 (26.5\%)}. An analysis of individual tasks reveals specialized strengths across models. Sora-2 excels at geometric construction tasks like \textbf{Ray Intersection (a remarkable 88\%)} and \textbf{Circle Center (70\%)}. In contrast, Claude 4.5 leads on a different set of tasks, including {Square Outlier (86\%)} and {Midpoint (66\%)}. In summary, while Sora-2's dynamic video output gives it the best overall performance, other models exhibit competitive strengths in specific areas of spatial reasoning.  

\input{table/b_eyeballing-tasks}

\begin{tcolorbox}[
    colback=blue!10,
    colframe=blue!50,
    boxrule=1pt,
    arc=3mm,
    left=5pt,
    right=5pt,
    top=5pt,
    bottom=5pt
]

\textbf{Takeaway 1} \quad Sora-2 generally \textbf{surpasses SOTA VLMs} on eyeballing puzzles. Sora-2 exhibits \textbf{geometric and physical} reasoning abilities. It can simulate the extension and reflection of rays and manipulate geometric elements (e.g., points and lines) to support spatial reasoning.
\end{tcolorbox}

\subsubsection{Visual Puzzles: Sora-2 has inductive reasoning capability}
\label{sec:visual_puzzles}

\textbf{Dataset Construction}

To evaluate \textbf{inductive reasoning capability} of video generation models such as Sora-2, we constructed \textbf{visual puzzle tasks} centered on pattern recognition and matching, as illustrated in Figure~\ref{fig:visual_puzzles}. Specifically, we transformed ten types of puzzles selected from PuzzleVQA~\citep{chia2024puzzlevqa} to video generation tasks, prompting the model to solve the visual puzzle via the generated video without giving the original multiple-choice options. We also modified the data generation code to produce the solution images along with the puzzles and introduced variations to diversify samples for some tasks. Each task contains around fifty samples.

As illustrated in Figure~\ref{fig:visual_puzzles}, the ten tasks are broadly categorized as follows:
\begin{itemize}[leftmargin=*]
    \item \textbf{Color-filling tasks} primarily requires the model to \textbf{fill the marked area with the correct color} (Tasks 1-6).
    \item \textbf{Shape-drawing tasks} primarily requires the model to \textbf{draw the correct shape} of the correct size in the marked area (Tasks 7-10).
\end{itemize}

\begin{figure*}[t]
\centering 
\includegraphics[width=\textwidth]{img/visual_puzzles/visual_puzzles_main.pdf}
\caption{\textbf{Overview of the visual puzzles}, categorized into color-fillings tasks and shape-drawing tasks. The tasks are selected and adapted from PuzzleVQA~\citep{chia2024puzzlevqa} to evaluate \textbf{inductive reasoning} capability. The video generation model need to fill the marked area with the correct color or draw the correct shape. Sora-2 correctly solved the problems above.}
\label{fig:visual_puzzles}
\end{figure*}

\textbf{Evaluation Setup}

\begin{itemize}[leftmargin=*]
    \item \textbf{Definition of Deviation Value}\quad We define a metric, denoted as \textit{Diff}, to \textbf{quantify the deviation} between a generated video frame and the solution image. It sums up the pixel-wise differences within the puzzle area. For color-filling tasks, the difference is based on color distance in RGB space; for shape-drawing tasks, it measures the pixel-wise mismatch. The formal definitions are provided in Appendix~\ref{app:visual_puzzle_diff}.
    
    \item \textbf{Best Frame Selection and Evaluation}\quad We selected \textbf{the ``best'' frame}, namely the frame with the lowest \textit{Diff} value. Sora-2 might generate unrelated content after task completion, or the target color/shape might appear gradually. So using the ``best'' frame helps determine the answer given in the video. We \textbf{manually} evaluated Sora-2's performance based on the ``best'' frames. \textbf{For the VLMs}, we provided them with multiple-choices in certain tasks and employed a rule-based evaluation, as detailed in Appendix~\ref{app:visual_puzzle_eval} and Appendix~\ref{app:visual_puzzle_prompts}.
\end{itemize}

\textbf{Evaluation Results}

\begin{itemize}[leftmargin=*]
    \item \textbf{Sora-2 demonstrates a certain level of inductive reasoning capability.} As shown in Table~\ref{tab:visual_puzzle_result}, Sora-2 performs strongly on certain tasks, such as Hexagon Color Pattern Matching \textbf{(96\%)} in color-filling tasks and Grid Size Pattern Matching \textbf{(85.4\%)} in shape-drawing tasks. The task examples are illustrated in Figure~\ref{fig:visual_puzzles}. These demonstrate Sora-2's capacity to identify the patterns to solve the puzzles.
    
    \item \textbf{Sora-2's performance is relatively close to certain SOTA VLMs.} Overall, Sora-2 does not perform as well as the three SOTA VLMs. However, the gap is not large in certain cases. For instance, on color-filling tasks, Sora-2 scores \textbf{67.0\%} on average, while Gemini 2.5 Pro scores \textbf{73.9\%}. Notably, Sora-2 averages \textbf{64.9\%} on shape-drawing tasks, close to \textbf{68.6\%} that Claude 4.5 Sonnet achieves, which is provided with multiple-choice options, illustrated in Figure~\ref{fig:visual_puzzle_sora_VLM_test_form_cmp}. These indicate Sora-2 holds potential in inductive reasoning.
\end{itemize}

\begin{tcolorbox}[
    colback=blue!10,        % 背景颜色（浅蓝色）
    colframe=blue!50,       % 边框颜色（深蓝色）
    boxrule=1pt,           % 边框粗细
    arc=3mm,               % 圆角
    left=5pt,              % 左边距
    right=5pt,             % 右边距
    top=5pt,               % 上边距
    bottom=5pt             % 下边距
]
%Sora-2在的颜色和形状两个维度，展现出总结规律与模式识别的能力用于求解puzzle，包括对称性（Grid Size Pattern Matching），连续性（Color Gradient Perception & Application），组合性（Color Mixing Perception & Application）
\textbf{Takeaway 2} \quad Sora-2’s performance is comparable to that of Claude Sonnet 4.5 on Shape-Drawing puzzles, demonstrating a certain level of \textbf{inductive reasoning} capability. Moreover, Sora-2 demonstrates the ability to recognize and apply \textbf{patterns of color, shape and size}. Sora-2 can solve visual puzzles patterns including \textbf{symmetry, gradients, and compositionality}.
\end{tcolorbox}

\input{table/c_visual-puzzle-tasks}

\begin{figure*}[h]
    \centering 
    \includegraphics[width=\textwidth]{img/arcagi2.pdf}
    \caption{\textbf{Examples of Sora-2 trying to solve ARC-AGI-2.} ARC-AGI-2 is a benchmark targeting few-shot, inductive reasoning over abstract pattern transformations. Sora-2 is expected to deduct the transform rule from examples and use the rule to generate the output grid of the test case. Besides automatic evaluation, we manually analyzed 100 cases and divide them into 4 categories based on completion level. Prompt: \textit{``Each row contains input and output grids. Learn the pattern and generate the output grid for the last input while keeping existing patterns without modification.  Static camera perspective, no zoom or pan. In portrait.``} For the generated video and ground truth, only test case area is displayed. Details: Section~\ref{sec:arc_agi_2}}
    \label{fig:case_arcagi2}
\end{figure*}


\subsubsection{ARC-AGI-2: Sora-2 is a few-shot learner}
\label{sec:arc_agi_2}
\textbf{Dataset Construction}


ARC-AGI-2~\citep{chollet2025arcagi2newchallengefrontier} is a benchmark targeting few-shot, inductive reasoning over abstract pattern transformations. Each piece of data includes several input grids and corresponding output grids, with a consistent rule of transformation between each input and output.
We use the 1000-sample ARC-AGI-2 train set. The original data is in json format, so we wrote a program to display each sample and pad the image to the same aspect ratio as Sora-2, while leaving last output grid as empty for Sora-2 to put its answer. We evaluate SOTA VLMs using the same image input and text instruction. We then compare their output color matrix (in text form) with the ground truth matrix.

For VLMs, we also show images instead of text matrixes for fair comparison. 

\textbf{Evaluation Setup}

A program automatically extracts last frame of video generated by Sora-2, zoom it into the size of input image, and calculate the average color of each cell. ARC-AGI-2 has a fixed 10 color palette, so for each cell, we check if the nearest color in the palette matches ground truth color. The answer is correct only if all cells are correct.

Besides automatic evaluation, we manually analyze randomly chosen 100 cases, and divide them into 4 categories, for more elaborate evaluation:
\begin{itemize}
    \item \textbf{Fully Correct:} All cells in the output grid are correct.
    \item \textbf{Mostly Correct:} The output grid shows understanding of the transformation rule, but has flaws on the details.
    \item \textbf{Partially Correct:} The output grid shares some characteristics with ground truth, but not enough to show Sora-2 understands the transformation rule.
    \item \textbf{Wrong:} The output grid is not related to the answer at all. ``Did Nothing'' is a subcategory that means the video does not modify the output area.


\end{itemize}

\textbf{Evaluation Results}

Sora-2 scores 1.3\%, which is on par with strong LLMs like Gemini 2.5 Pro and GPT5 high. This indicates Sora-2 has developed elementary abstract reasoning.

The Fully Correct case in Fig.~\ref{fig:case_arcagi2} further suggests a capacity of self-correction, rather than a single-shot pattern guess. In the first middle frame, three green pixels in the bottom right forming ``V'' shape are misplaced 1 pixel upward. This mistake is corrected in the next frame, leading to the correct final answer. 

The manual analyze result is shown in Table~\ref{tab:arcagi_manual}. While the ``Fully Correct'' rate of 3\% is low, the 14 ``Mostly Correct'' outputs indicate that the model can sometimes identify the core transformation rule has problems with execution. A significant portion of failures (42 out of 55) were instances where the model ``Did Nothing'', that is not changing the output area during the video. A proportion of them change the test case input area or few shot examples area instead, showing struggles with understanding the instruction.

\begin{tcolorbox}[
    colback=blue!10,        % 背景颜色（浅蓝色）
    colframe=blue!50,       % 边框颜色（深蓝色）
    boxrule=1pt,           % 边框粗细
    arc=3mm,               % 圆角
    left=5pt,              % 左边距
    right=5pt,             % 右边距
    top=5pt,               % 上边距
    bottom=5pt             % 下边距
]

 

\textbf{Takeaway 3} \quad In-context learning (ICL) is a paradigm for natural language processing (NLP), where LLMs make predictions based on contexts augmented with a few examples. We find \textbf{Sora-2 is a few-shot learner}. We evaluate it on ARC-AGI-2, which requires the model to find patterns in given input-output pairs and apply these patterns to new inputs. While SOTA VLMs struggle on ARC-AGI-2 and achieve less than 5\% accuracy, we observe that Sora-2 can often make \textbf{reasonable predictions}, although they do not strictly match the dataset annotations.
\end{tcolorbox}

\begin{table}[t]
    \centering
    \small
    \setlength{\tabcolsep}{6pt}
    \begin{tabular}{lcccc}
        \toprule
        \multirow{2}{*}{\textbf{Task}} & \multirow{2}{*}{\textbf{Sora-2}} & \textbf{Gemini} & \textbf{GPT5} & \textbf{Claude} \\
         & & \textbf{2.5 Pro} & \textbf{high} & \textbf{Sonnet 4.5} \\
        \midrule
        ARC-AGI-2 & 1.3 & 1.9 & 0.5 & 5.3 \\
        \bottomrule
    \end{tabular}
    \caption{Accuracy (\%) on the ARC-AGI-2 task. We display each sample in an image and send it to Sora-2 and VLMs. Details: Sec.~\ref{sec:arc_agi_2}}
    \label{tab:arcagi_leaderboard_transposed}
\end{table}




==> old/section/evaluation/c_text.tex <==
\subsection{Text-Centric Reasoning Tasks}
\label{sec:text-centric_reasoning_task}

\begin{figure*}[t]
\centering 
\caption{Input form and evaluation of text-centric tasks. The model accepts a text prompt and a reference image. The prompt contains the problem text and the reference image displays the entire problem. The model shows the textual solution process and the answer in the video, speaking the answer in the audio. We evaluate the answers from the video and audio \textbf{independently}. The last frame is extracted for video evaluation and the audio is transcribed for audio evaluation. For evaluation, we adopt an LLM-as-a-Judge approach, detailed in Section~\ref{sec:text-centric_eval}, and human alignment check is shown in Appendix~\ref{app:human_alignment_text}.}
\includegraphics[width=\textwidth]{img/text-centric_main.png}
\vspace{-20pt}
\label{fig:text-centric_eval_pipeline}
\end{figure*}

\subsubsection{Dataset Construction}
\label{sec:text-centric_data_construction}

\paragraph{Using Subsets of Selected Benchmarks}

The text-centric tasks are adapted from established benchmarks. For evaluation cost control, we \textbf{sampled a subset} for most of the benchmarks instead of using the full test set, with statistics shown in Appendix~\ref{app:bench_sample_distribution}. Below are the selected benchmarks.

\begin{itemize}[leftmargin=*]
    \item \textbf{Text-Only Reasoning Benchmarks}\quad We evaluate math reasoning abilities using the three representative math reasoning benchmarks of increasing difficulty: GSM8K~\citep{cobbe2021gsm8k}, MATH-500~\citep{cobbe2021training} and AIME of year 2024 and 2025. For general knowledge reasoning evaluation, we select BBH~\citep{suzgun2022challengingbigbenchtaskschainofthought}, MMLU~\citep{hendrycks2020measuring}, MMLU-Pro~\citep{wang2024mmlu}, GPQA-diamond~\citep{rein2024gpqa} and SuperGPQA-easy~\citep{du2025supergpqa}.
    
    \item \textbf{Multimodal Reasoning Benchmarks}\quad We select MathVista~\citep{lu2023mathvista} and MathVision~\citep{wang2024measuring} to evaluate multimodal math reasoning abilities, and use MMBench~\citep{liu2024mmbench} and MMMU~\citep{yue2024mmmu} which assess general visual understanding and multi-discipline multimodal reasoning, respectively.
\end{itemize}

\paragraph{Input Form and Instruction} We use both \textbf{a text prompt} and \textbf{a reference image} for text-centric tasks. As shown in Fig.~\ref{fig:text-centric_eval_pipeline}, text prompt  contains the full problem text for text-only problems or the textual component for multimodal problems. The reference image displays the entire problem on a white background. The problem text is in printed form. For multimodal problems, the original image is embedded. The model provides a \textbf{written solution process and the answer} within the video. In the audio track, it should only state the final answer without any explanation, to avoid truncation due to video length constraints.
    
\subsubsection{Evaluation Setup}
\label{sec:text-centric_eval}

\paragraph{Video and Audio Evaluation} We evaluate the answers from the video and audio \textbf{independently}. The \textbf{last frame} of each video, is used for video evaluation. The audio is \textbf{transcribed into text} for audio evaluation. We report accuracies for video and audio, along with the rate at which answers are correct in \textbf{both modalities (denoted V $\cap$ A)} and in \textbf{at least one modality (denoted V $\cup$ A)}.
    
\paragraph{LLM as a Judge} We adopt an LLM-as-a-Judge~\citep{zheng2023judging} approach for video and audio evaluation, using GPT-4o~\citep{openai2024gpt4o} as the judge model. The model is given the last frame image (for video) or the transcribed text (for audio), with the evaluation prompts shown in Appendix~\ref{app:eval_prompt_text-centric}. Human alignment check shown in Appendix~\ref{app:human_alignment_text} validates the evaluation.
    
\subsubsection{Evaluation Results}
\label{sec:text_centric_eval_results}

The evaluation results for text-only and multimodal reasoning problems in text-centric tasks are presented in Table~\ref{tab:text_centric_reasoning_statistics}. Notably, Sora-2 \textbf{shows surprising performance on text-centric tasks}. In terms of audio accuracy, Sora-2 achieves performance \textbf{comparable to SOTA VLMs} on several datasets across both text-only and multimodal reasoning ones, such as GSM8K, MATH-500, and MathVista. Although a noticeable gap remains between Sora-2 and SOTA VLMs on more challenging datasets like AIME, GPQA, and MMMU, Sora-2 overall demonstrates potential in text-centric reasoning tasks. Besides, it is observed that Sora-2's \textbf{audio accuracy is higher than video accuracy}. Sora-2 achieves consistently higher accuracies in audio than in video across most datasets, spanning text-only and multimodal reasoning problems. This may be attributed to Sora-2's difficulty in generating accurate written content, which is analyzed in Section~\ref{sec:text_reason_process}.

\input{table/e_text-centric-tasks}

\begin{tcolorbox}[
    colback=blue!10,
    colframe=blue!50,
    boxrule=1pt,
    arc=3mm,
    left=5pt,
    right=5pt,
    top=5pt,
    bottom=5pt
]
\textbf{Takeaway 4} \quad On text-centric tasks, Sora-2 shows surprising performance on text and multimodal reasoning tasks. The video generation model is able to \textbf{embed text within video frames}, enabling unified multimodal understanding and generation. Thus, ``Thinking with Video'' is potentially a \textbf{unified multimodal reasoning paradigm}.
\end{tcolorbox}

==> old/section/experiment/a1_output_form_self_consistency.tex <==
\input{table/f_g_arc-fewshot}

\subsubsection{Self-Consistency Improves Video Generation Reasoning}
\label{sec:self_consistency}

Self-consistency relies on a key intuition. It is the idea that for a complex reasoning problem, there are multiple valid ways to think about it. All these \textbf{different paths} can ultimately lead to the same \textbf{unique correct answer} \citep{wang2023selfconsistencyimproveschainthought}. The results in Table~\ref{tab:output_modality_results} demonstrate a principle similar to ``self-consistency'' in large language models. This principle is evident when comparing the Last Frame Option with the Major Frame Option.

The accuracy improves from 56\% for the single Last Frame Option analysis to 68\% for the time-averaged Major Frame Option. This initial improvement suggests that analyzing Sora-2's output over time provides a more robust measure of its intent. Upon inspection, we find that the end of generated videos sometimes flash to SMPTE color bars or pure black screen, leading to failure of last frame image. By sampling across the video's duration, the Major Frame Option method effectively acts as a denoising filter, capturing the model's most consistent and stable belief about the correct answer.

This effect is magnified when considering the majority vote over five retries. While the Last Frame Option accuracy improves from 56\% to 66\% with voting, the Major Frame Option accuracy leaps from 68\% to an impressive 90\%. This demonstrates that the temporal consistency within a single video is a strong proxy for the model's confidence. When this temporally consistent signal is further aggregated across multiple independent generation attempts, the result is a highly reliable extraction of the model's core reasoning capability. The model, when it understands the problem, will consistently generate videos where the indicator remains on the correct option over time and across multiple attempts. This temporal self-consistency provides a much more accurate assessment of the model's problem-solving abilities than an evaluation based on a single, static final output.

\begin{tcolorbox}[
    colback=blue!10,
    colframe=blue!50,
    boxrule=1pt,
    arc=3mm,
    left=5pt,
    right=5pt,
    top=5pt,
    bottom=5pt
]
%以Self-consistency为代表的Test time scaling在文本推理任务上取得巨大成功
\textbf{Takeaway 6} \quad Test time scaling methods, represented by Self-consistency, have achieved great success in text reasoning tasks. We find that \textbf{self-consistency} can \textbf{improve} Sora-2’s performance in the verifiable video generation reasoning task. This reveals an
underexplored direction: \textbf{test time scaling in video generation reasoning tasks}.
\end{tcolorbox}

==> old/section/experiment/a2_fewshot.tex <==
\subsubsection{Sora-2's in-context learning improves with more examples}
\label{sec:sora_few_shot}

Each sample in ARC-AGI-2 has multiple demonstration examples. To test Sora-2's few-shot learning capabilities, we conducted an experiment where we provided only a single example (1-shot) instead of all available examples, and retested Sora-2 on the 1000 training samples. Since achieving a perfectly correct grid is difficult, we measure performance using "pixel accuracy": the percentage of pixels in the output area that match the ground truth. The results, comparing performance with all examples versus just one, are presented in Table~\ref{tab:pixel_accuracy_ranges}.

The results show a clear trend. Comparing to using all examples, \textbf{1-shot yields more low-accuracy (0 to 0.35) samples} and \textbf{less high-accuracy (0.65 to 1.0) samples,}. This demonstrates that while Sora-2 has some 1-shot ability, its performance on this abstract reasoning task benefits from seeing multiple examples, confirming it as a few-shot learner.

\begin{tcolorbox}[
    colback=blue!10,
    colframe=blue!50,
    boxrule=1pt,
    arc=3mm,
    left=5pt,
    right=5pt,
    top=5pt,
    bottom=5pt
]



\textbf{Takeaway 5} \quad Sora-2 can achieve better in-context learning by providing more examples. Experiments show that Sora-2 performs better when provided with all examples, compared to only one example. This is an underexplored direction for analyzing and improving the in-context learning abilities of video generation models.
\end{tcolorbox}

==> old/section/experiment/b1_testset_leakage.tex <==
\subsubsection{Test Set Leakage Analysis}
\label{sec:exp_leakage}

To investigate potential test data leakage as the reason for Sora-2's strong performance in text-centric reasoning, we further \textbf{create new evaluation problems} from the math reasoning test data. Specifically, we used Qwen3-235B-A22B-Thinking-2507~\citep{yang2025qwen3} and Gemini 2.5 Pro~\citep{comanici2025gemini} to generate similar problems for problems of our GSM8K and MATH-500 test data, respectively, with the prompts shown in Appendix~\ref{app:data_leakage_prompt}. Each newly generated problem shares the same the underlying problem-solving structure as its original counterpart but \textbf{features different numerical values} and possibly different contextual details.

We evaluated Sora-2 on these derived problems and found \textbf{no significant performance difference} compared to the original problems, as shown in Table~\ref{tab:test_leakage_analysis}. This consistency suggests that Sora-2's performance \textbf{stems from its inherent text-centric reasoning capabilities} rather than test data leakage.

\begin{table}[t]
    \centering
    \small
    \setlength{\tabcolsep}{9pt}
    \begin{tabular}{lcccc}
        \toprule
        \textbf{Dataset} & \textbf{Last Frame} & \textbf{Audio} & \textbf{V $\cap$ A} & \textbf{V $\cup$ A} \\
        \midrule
        GSM8K & 75.7 & 98.9 & 75.7 & 98.9 \\
        GSM8K (Derived) & 78.4 & 100.0 & 78.4 & 100.0 \\
        \midrule
        MATH-500 & 67.0 & 92.0 & 65.0 & 94.0 \\
        MATH-500 (Derived) & 75.0 & 91.0 & 71.0 & 95.0 \\
        \bottomrule
    \end{tabular}
    \caption{Sora-2’s accuracy on original and derived math reasoning problems \textbf{with different numerical values}.  V $\cap$ A denotes the rate at which answers are correct in both video and audio. V $\cup$ A denotes the rate at which answers are correct in at least one of video and audio. \textbf{Performance remains consistent}, thus excluding the risk of test data leakage and indicating Sora-2's inherent potential in text-centric reasoning tasks. Human alignment check shown in Appendix ~\ref{app:human_alignment_text} validates the evaluation.}
    \label{tab:test_leakage_analysis}
\end{table}

==> old/section/experiment/b2_text_reason_process.tex <==
\subsubsection{Analysis of Sora-2's Reasoning Process}
\label{sec:text_reason_process}

To better understand Sora-2's text-centric reasoning, we sampled 115 cases from the problems that Sora-2 answered correctly via both video and audio across the text-centric tasks, and manually analyzed the generated reasoning processes. We categorized each case into five categories: (1) Completely Correct, (2) Logic Correct with Writing Errors, (3) Unreadable or Incorrect Logic, (4) Missing Solution Process, and (5) Process Unnecessary. Detailed definitions and examples are provided in Appendix~\ref{app:solution_process_categories}.

Our analysis reveals that Sora-2 \textbf{struggles to generate coherent reasoning processes} in the video, even when providing a correct final answer. As shown in Figure~\ref{fig:solution_pie_chart}, only 13.91\% of solutions are fully correct. The majority of solutions (43.48\%) are \textbf{unreadable or logically flawed}, with another 29.57\% containing minor presentation errors. This suggests that Sora-2 has major difficulties in delivering a clear and correct reasoning process via video generation.

==> old/section/experiment/b4_source_text_reason_ability.tex <==
\subsubsection{Source of Text-Centric Reasoning Ability}
\label{sec:source_text_reasoning_ability}

Despite Sora-2's strong text-centric reasoning (Section~\ref{sec:text_centric_eval_results}), its video generation pipeline might contain \textbf{a prompt rewriter model} that solves the problems for the video generation component. Since Sora-2 \textbf{lacks controllable prompt rewriting for users}, we used Wan2.5~\citep{wan2025wan}, which provides a parameter (\texttt{prompt\_extend}) for enabling/disabling its rewriting behavior. We then evaluated Wan2.5 (wan2.5-i2v-preview) under both settings on the sampled subsets of GSM8K, MMLU and MMMU, using generally the same setup as for Sora-2.

As shown in Table~\ref{tab:wan2.5_text_reason_test}, \textbf{Wan2.5 achieves nearly zero accuracy} across all three text-centric benchmarks when its prompt rewriter is disabled. In contrast, enabling prompt rewriting leads to a substantial performance gain. This significant gap demonstrates that Wan2.5's text-centric reasoning ability is almost entirely from its prompt rewriter model. A concrete example illustrating how prompt rewriting transforms a reasoning problem into explicit visual instructions is provided in Appendix~\ref{app:wan_prompt_rewrite_case}. This suggests that the strong text-centric reasoning capability observed in Sora-2 may also \textbf{stem from an internal prompt rewriting mechanism}, possibly using a VLM.

\begin{tcolorbox}[
    colback=blue!10,
    colframe=blue!50,
    boxrule=1pt,
    arc=3mm,
    left=5pt,
    right=5pt,
    top=5pt,
    bottom=5pt
]
%Sora-2在Text-Centric Reasoning Tasks 上取得了惊人的结果。我们通过实验分析了Sora-2的能力来源。Sora-2在改编数学问题上保持和原测试集相近性能。此结果降低了测试集泄露的可能性。我们分析了Sora-2的推理过程，发现Sora-2 struggles to generate coherent reasoning processes in the video, even when providing a correct final answer. 最终通过对Wan 2.5的对比实验，我们推测Sora-2的Text-Centric Reasoning能力来源于提示词改写器。
\textbf{Takeaway 7} \quad Sora-2 has achieved impressive results on Text-Centric Reasoning Tasks. We conducted experiments to analyze \textbf{the source of Sora-2's capabilities}. Sora-2 maintains performance comparable to the original test set on adapted math problems, which reduces the likelihood of test set leakage. We also analyzed Sora-2's reasoning process and found that it struggles to generate coherent reasoning steps in the video, even when providing the correct final answer. Finally, through comparative experiments with Wan 2.5, we speculate that Sora-2's Text-Centric Reasoning ability originates from its \textbf{prompt rewriter}.
\end{tcolorbox}

\begin{figure}[t]
    \begin{minipage}[t]{0.55\textwidth}
        \centering
        \includegraphics[valign=t, width=0.9\textwidth]{img/solution_process_pie_chart.pdf}
        \caption{Distribution of reasoning process categories for correct answers. The prevalence of ``Unreadable or Incorrect Logic'' \textbf{(43.48\%)} highlights Sora-2's difficulty in generating coherent reasoning.}
        \label{fig:solution_pie_chart}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.43\textwidth}
        \centering
        \small
        \setlength{\tabcolsep}{3pt}
        \vspace{1.5mm}
        \begin{tabular}{cccccc}
            \toprule
            \textbf{Dataset} & \makecell{\textbf{Prompt} \\ \textbf{Rewrite}} & \makecell{\textbf{Last} \\ \textbf{Frame}} & \textbf{Audio} & \textbf{V $\cap$ A} & \textbf{V $\cup$ A} \\
            \midrule
            \multirow{2}{*}{GSM8K} & \xmark & 0.0 & 0.0 & 0.0 & 0.0 \\
             & \cmark & \textbf{78.4} & \textbf{31.9} & \textbf{29.2} & \textbf{81.6} \\
            \midrule
            \multirow{2}{*}{MMLU} & \xmark & 0.0 & 0.0 & 0.0 & 0.0 \\
             & \cmark & \textbf{74.1} & \textbf{50.00} & \textbf{50.00} & \textbf{74.1} \\
            \midrule
            \multirow{2}{*}{MMMU} & \xmark & 2.0 & 0.0 & 0.0 & 2.0 \\
             & \cmark & \textbf{47.0} & \textbf{14.0} & \textbf{11.0} & \textbf{50.0} \\
            \bottomrule
        \end{tabular}
        \captionof{table}{Wan2.5's performance on text-centric tasks with and without prompt rewriting. Its reasoning ability almost vanishes when the prompt rewriter model is disabled, indicating that this component solves the reasoning problems for the video generation component.  This suggests the strong text-centric reasoning capability observed in Sora-2 may also stem from a prompt rewriter model.}
        \label{tab:wan2.5_text_reason_test}
    \end{minipage}
\end{figure}

==> preamble.tex <==
%% This file contains a number of tweaks that are typically applied to the main document.
%% They are not enabled by default, but can be enabled by uncommenting the relevant lines.

%%
%% Inline annotations; for predefined colors, refer to "dvipsnames" in the xcolor package:
%% https://tinyurl.com/overleaf-colors
%%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
%%
%% disable for camera ready / submission by uncommenting these lines  
%%
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}

%%
%% work harder in optimizing text layout. Typically shrinks text by 1/6 of page, enable
%% it at the very end of the writing process, when you are just above the page limit
%%
% \usepackage{microtype}

%%
%% fine-tune paragraph spacing
%%
% \renewcommand{\paragraph}[1]{\vspace{.5em}\noindent\textbf{#1.}}

%%
%% globally adjusts space between figure and caption
%%
% \setlength{\abovecaptionskip}{.5em}


%%
%% Allows "the use of \paper to refer to the project name"
%% with automatic management of space at the end of the word
%%
% \usepackage{xspace}
% \newcommand{\paper}{ProjectName\xspace}

%%
%% Commonly used math definitions
%%
% \DeclareMathOperator*{\argmin}{arg\,min}
% \DeclareMathOperator*{\argmax}{arg\,max}

%%
%% Tigthen underline
%%
% \usepackage{soul}
% \setuldepth{foobar}


% --- For Math and Symbols ---
\usepackage{amsfonts}       % Blackboard math symbols
\usepackage{nicefrac}       % Compact symbols for 1/2, etc.
\usepackage{pifont}         % For checkmarks (\ding)

% --- For Figures and Subfigures ---
\usepackage{subcaption}     % For subfigures
\usepackage[export]{adjustbox} % For fine-tuning figure alignment/size

% --- For Tables ---
\usepackage{booktabs}       % Professional-quality tables (\toprule, \midrule, \bottomrule)
\usepackage{multirow}       % For multi-row cells in tables
\usepackage{makecell}       % For multi-line cells and better vertical spacing
\usepackage{tabularx}       % For tables with auto-adjusting columns
\usepackage{array}          % For advanced column formatting in tables
\usepackage{siunitx}        % For better number alignment in tables

% --- For Plots and Drawings ---
\usepackage{tikz}
\usepackage{pgfplots}
\pgfplotsset{compat=1.17}   % Good practice to set a compatibility version for pgfplots
\usepackage{pgf-pie}        % For creating pie charts with pgf/tikz

% --- Utilities and Styling ---
\usepackage{xcolor}         % For defining and using colors (essential for your commands)
\usepackage{enumitem}       % For customizing lists (itemize, enumerate)
\usepackage{comment}        % For using \begin{comment} ... \end{comment} blocks

% --- Packages to Use with Caution ---
\usepackage{wrapfig}        % For wrapping text around figures. Can be tricky in two-column format.
\usepackage{tcolorbox}      % Main package for colored boxes
\tcbuselibrary{breakable}    % Allows tcolorboxes to break across pages
\tcbuselibrary{skins}        % Provides advanced styling for tcolorboxes

% --- IMPORTANT: The CVPR template handles hyperref. Do NOT add \usepackage{hyperref} here. ---
% It will be included automatically by the cvpr.cls file with the correct options.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% --- YOUR CUSTOM COMMANDS AND DEFINITIONS (migrated from the old template) ---
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% --- Custom Colors ---
\definecolor{lightblue}{RGB}{200, 230, 255}
\definecolor{headerblue}{RGB}{150, 200, 255}
\definecolor{ForestGreen}{RGB}{34, 139, 34}
\definecolor{Red}{RGB}{255, 0, 0}
\definecolor{tickG}{rgb}{0.1, 0.588, 0.1}
\definecolor{crossR}{rgb}{0.588, 0.1, 0.1}
\definecolor{frenchblue}{rgb}{0.0, 0.45, 0.73}
\definecolor{babyblue}{rgb}{0.54, 0.81, 0.94}
\definecolor{classicrose}{rgb}{0.98, 0.8, 0.91}
\definecolor{beige}{rgb}{0.96, 0.96, 0.86}
\definecolor{forestgreen}{HTML}{2e7d43}
\definecolor{blue1}{HTML}{91BBE6}
\definecolor{blue2}{HTML}{3F90E0}
\definecolor{blue3}{HTML}{316FAD}
\definecolor{color1}{HTML}{FF9999}
\definecolor{color2}{HTML}{FF6666}
\definecolor{color3}{HTML}{FF3333}
\definecolor{color4}{HTML}{E60000}
\definecolor{color5}{HTML}{B30000}
\definecolor{color6}{HTML}{8CD98C}
\definecolor{color7}{HTML}{53c653}
\definecolor{color8}{HTML}{00B050}
\definecolor{color9}{HTML}{2d862d}
\definecolor{color10}{HTML}{206020}
\definecolor{color11}{HTML}{cca300}

% --- Custom Box Environment ---
\newtcolorbox{promptbox}[2][]{
    colback=white,
    coltext=black,
    arc=3mm,
    boxrule=0.5pt,
    colframe=black!60!white,
    title={#2},
    colbacktitle=black,
    coltitle=white,
    fonttitle=\bfseries,
    top=8pt,
    bottom=8pt,
    left=10pt,
    right=10pt,
    breakable,
    before upper={%
        \linespread{1}\selectfont
        \setlength{\parskip}{1ex plus 0.2ex minus 0.2ex}
        \setlength{\parindent}{0pt}
    },
    #1
}

% --- Custom Macros for Content ---
\newcommand{\maxbold}[1]{\textbf{#1}}
\newcommand{\cmark}{\textcolor{tickG}{\ding{52}}}   % checkmark
\newcommand{\xmark}{\textcolor{crossR}{\ding{56}}}   % cross mark

% --- Macros for Tables ---
\newcommand{\catA}{\makecell{3D Spatial \\ Perc. \& Under.}}
\newcommand{\catB}{\makecell{Pattern Recog. \\ \& Matching}}
\newcommand{\catC}{\makecell{Multi-step \\ Reasoning}}
\newcommand{\catD}{\makecell{Strategic \\ Planning}}

% --- Macros for Plots ---
\def\axisLabels{{CharXiv, MMBench, MMMU, MMMU-Pro, MathVerse, MathVision, MathVista}}
% \setlength\parindent{0pt}

% 目录
\usepackage{titletoc}

% % 引入 multibib 包
% \usepackage{multibib}
% % 定义一个新的引用类别，名字叫 'supp'
% % 第二个参数是该参考文献列表的标题，例如 "References" 或 "Supplementary References"
% \newcites{supp}{Supplementary References}

\usepackage{tocloft}
\setlength{\cftsubsecindent}{1em} 
\setlength{\cftsubsubsecindent}{2em} 


==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets the figure captions and references in a smaller font.
The reason why such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The review process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in 11 pages.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler that should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use the options of \texttt{cvpr.sty} to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Use fractional references (\eg, this line is $087.5$), although in most cases the approximate location would be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please, number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for the reader to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean that some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not mean that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper, we present a performance analysis of our previous paper [1], and show that it is inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper, we present a performance analysis of the paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time that covers similar or overlapping material, you may need to refer to that submission to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, do not assume that the reviewers will read this material.

Sometimes your paper is about a problem that you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think that it is likely that the new article was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
However, for your results, you should not identify yourself and should not mention your participation in the challenge.
Instead, present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison with other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has only two authors.

\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}


==> sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
The columns should be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered, and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

The captions of the figures and tables should be in 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centered.  Table captions should be above tables, while figure captions should be below figures.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period, and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use the footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example, at the beginning of the sentence, you can use
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, include the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When citing multiple papers at once, make sure that you cite them in numerical order such as this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \caption{Results.   Ours is better.}
  \label{tab:example}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead, use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise and, therefore, must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it is almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence, avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> table/b_eyeballing-tasks.tex <==
\newcolumntype{C}{>{\centering\arraybackslash}X}
\begin{table*}[ht]
    \centering
    \caption{Accuracy (\%) of Sora-2 using 3 evaluation methods and 3 VLMs on eyeballing tasks. The highest score in each row is highlighted in bold. For Sora-2, answers are derived from its generated audio (transcribed), the final video frame (which option is closest to red dot location), or by a majority vote across multiple frames. VLM answers are extracted from their text output. We divide tasks into three categories based on whether it constructs a point, a line or a shape. Details: Section~\ref{sec:spatial_reasoning}}
    \label{tab:spatial_reasoning_results}
    \small
    \setlength{\tabcolsep}{2pt} % Adjust column spacing for better fit
    \begin{tabularx}{\linewidth}{lCCCCCC}
    \toprule
    \multirow{2}{*}{\textbf{Task}} & \textbf{Sora-2} & \textbf{Sora-2} & \textbf{Sora-2} & \textbf{Gemini} & \textbf{GPT5} & \textbf{Claude} \\
    &\textbf{Audio}&\textbf{Last Frame}&\textbf{Major Frame}&\textbf{2.5 Pro}&\textbf{high}&\textbf{Sonnet 4.5}\\
    \midrule
    \multicolumn{7}{c}{\textit{Point Tasks}} \\
    % \midrule
    Circle Center          & 58.0 & 56.0 & \textbf{70.0} & 44.0 & 62.0 & 50.0 \\
    Circumcenter           & 14.0 & 20.0 & 24.0 & 12.0 & \textbf{32.0} & 26.0 \\
    Fermat Point           & 24.0 & 24.0 & 30.0 & 30.0 & 28.0 & \textbf{34.0} \\
    Incenter               & \textbf{48.0} & 30.0 & 34.0 & 32.0 & 30.0 & 34.0 \\
    Midpoint               & 22.0 & 48.0 & 64.0 & 28.0 & 34.0 & \textbf{66.0} \\
    Orthocenter            & \textbf{32.0} & 18.0 & 26.0 & 14.0 & \textbf{32.0} & 28.0 \\
    Point Reflection       & 18.0 & 22.0 & 22.0 & \textbf{30.0} & 28.0 & \textbf{30.0} \\
    Ray Intersection       & 22.0 & 70.0 & \textbf{88.0} & 22.0 & 16.0 & 22.0 \\
    Triangle Center        & 34.0 & 42.0 & \textbf{44.0} & 38.0 & 40.0 & 36.0 \\
    % \midrule
    \textbf{Average}       & 30.2 & 36.7 & \textbf{44.7} & 27.8 & 33.6 & 36.2 \\
    \midrule
    \multicolumn{7}{c}{\textit{Line Tasks}} \\
    % \midrule
    Angle Bisector         & 28.0 & 36.0 & \textbf{38.0} & 28.0 & 28.0 & 24.0 \\
    Arc Connect            & 12.0 & 56.0 & \textbf{68.0} & 20.0 & 20.0 & 12.0 \\
    Circle Tangent Line    & 22.0 & 20.0 & \textbf{26.0} & 22.0 & 20.0 & 22.0 \\
    Circle Tangent Point   & 18.0 & 16.0 & \textbf{24.0} & 22.0 & 18.0 & 22.0 \\
    Parallel               & 22.0 & 28.0 & 30.0 & 20.0 & \textbf{32.0} & \textbf{32.0} \\
    Perpendicular          & 20.0 & 38.0 & \textbf{46.0} & 8.0  & 26.0 & 14.0 \\
    Perpendicular Bisector & 22.0 & 20.0 & 40.0 & 16.0 & 30.0 & \textbf{58.0} \\
    Ray Reflection         & 28.0 & 30.0 & \textbf{32.0} & \textbf{32.0} & 18.0 & 26.0 \\
    % \midrule
    \textbf{Average}       & 21.5 & 30.5 & \textbf{38.0} & 21.0 & 24.0 & 26.3 \\
    \midrule
    \multicolumn{7}{c}{\textit{Shape Tasks}} \\
    % \midrule
    Isosceles Trapezoid    & 36.0 & \textbf{42.0} & 36.0 & 24.0 & 26.0 & 20.0 \\
    Parallelogram          & 24.0 & 28.0 & 32.0 & 24.0 & 30.0 & \textbf{36.0} \\
    Right Triangle         & 30.0 & 14.0 & 16.0 & 38.0 & 20.0 & \textbf{60.0} \\
    Square Outlier         & 54.0 & 44.0 & 54.0 & 52.0 & 54.0 & \textbf{86.0} \\
    % \midrule
    \textbf{Average}       & 36.0 & 32.0 & 34.5 & 34.5 & 32.5 & \textbf{50.5} \\
    \midrule
    \textbf{Overall Average} & 28.0 & 33.4 & \textbf{40.2} & 26.5 & 29.7 & 35.1 \\
    \bottomrule
    \end{tabularx}
\end{table*}
